ATSim3D: Towards Accurate Thermal Simulator for Heterogeneous 3D-IC Systems Considering Nonlinear Leakage and Conductivity

Thermal simulation plays a fundamental role in the thermal design of integrated circuits, especially 3D ICs. Current simulators require significant runtime for high-resolution simulation, and dismiss the complex nonlinear thermal effects, such as nonlinear thermal conductivity and leakage power. To address these issues, we propose ATSim3D, a thermal simulator for simulating the steady-state temperature profile of nonlinear and heterogeneous 3D IC systems. We utilize the global-local approach, combining a compact thermal model at the global level, and a finite volume method at the local level. We tackle the nonlinear effects with Kirchhoff transformation and iteration. ATSim3D enables local-level parallelization that helps achieve an average speedup of 40x compared to COMSOL, with a relative error <3% and a state-of-the-art resolution of 4096 x 4096, holding promise for enhancing thermal-aware design in 3D ICs.

==> doc/abstract.tex <==
\begin{abstract}
Thermal simulation plays a fundamental role in the thermal design of integrated circuits, especially 3D ICs. Current simulators require significant runtime for high-resolution simulation, and dismiss the complex nonlinear thermal effects, such as nonlinear thermal conductivity and leakage power. To address these issues, we propose ATSim3D, a thermal simulator for simulating the steady-state temperature profile of nonlinear and heterogeneous 3D IC systems. We utilize the global-local approach, combining a compact thermal model at the global level, and a finite volume method at the local level. We tackle the nonlinear effects with Kirchhoff transformation and iteration. ATSim3D enables local-level parallelization that helps achieve an average speedup of 40× compared to COMSOL, with a relative error <3\% and a state-of-the-art resolution of 4096 × 4096, holding promise for enhancing thermal-aware design in 3D ICs.
\end{abstract}

\iffalse
\keywords{}
\fi

